A Unifying Perspective on Non-Stationary Kernels for Deeper Gaussian Processes

The Gaussian process (GP) is a popular statistical technique for stochastic function approximation and uncertainty quantification from data. GPs have been adopted into the realm of machine learning in the last two decades because of their superior prediction abilities, especially in data-sparse scenarios, and their inherent ability to provide robust uncertainty estimates. Even so, their performance highly depends on intricate customizations of the core methodology, which often leads to dissatisfaction among practitioners when standard setups and off-the-shelf software tools are being deployed. Arguably the most important building block of a GP is the kernel function which assumes the role of a covariance operator. Stationary kernels of the Mat\'ern class are used in the vast majority of applied studies; poor prediction performance and unrealistic uncertainty quantification are often the consequences. Non-stationary kernels show improved performance but are rarely used due to their more complicated functional form and the associated effort and expertise needed to define and tune them optimally. In this perspective, we want to help ML practitioners make sense of some of the most common forms of non-stationarity for Gaussian processes. We show a variety of kernels in action using representative datasets, carefully study their properties, and compare their performances. Based on our findings, we propose a new kernel that combines some of the identified advantages of existing kernels.

==> obsolete/obsoleteReview.tex <==
% The simple technique used in this paper is to measure non-stationarity in the covariance structure of a dataset based on the idea of model misspecification. 
% If we assume that the true generating model (i.e., data-generating
% mechanism that generates the training data) and the fitted GP model
% both belong to the same model class $\mathcal{M}$ parameterized by
% the likelihood family $p(\mathbf{y},\mathbf{x}\mid(\sigma_s,l))$, $(\sigma_s,l)$ is the stationary-kernel parameterization (the hyperparameters)
% of a stationary and isotropic GP, then minimizing the KL divergence is equivalent to maximizing
% the likelihood. Assuming the stationary data-generating model $p(\mathbf{y},\mathbf{x}\mid(\sigma_s,l)_{2})$
% and a stationary GP model likelihood $p(\mathbf{y},\mathbf{x}\mid(\sigma_s,l)_{1})$, the following
% argument shows this equivalence.
 
% \begin{align}(\sigma_s,l)^{*} & =\mathop{{\rm arg\,min}}\limits _{(\sigma_s,l)}D_{KL}(p(\mathbf{y},\mathbf{x}|(\sigma_s,l)_{1})||p(\mathbf{y},\mathbf{x}|(\sigma_s,l)_{2}))\\
%  & =\mathop{{\rm arg\,min}}\limits _{(\sigma_s,l)}E_{p(\mathbf{y},\mathbf{x}\vert(\sigma_s,l)_{1})}\left[\log p(\mathbf{y},\mathbf{x}\vert(\sigma_s,l)_{1})-\log p(\mathbf{y},\mathbf{x}\vert(\sigma_s,l)_{2})\right]\\
%  & =\mathop{{\rm arg\,max}}\limits _{(\sigma_s,l)}E_{p(\mathbf{y},\mathbf{x}\vert(\sigma_s,l)_{1})}\left[\log p(\mathbf{y},\mathbf{x}\vert(\sigma_s,l)_{2})\right]
% \end{align}
% Now, when the data-generating model and stationary GP models  don't belong
% to the same model class $\mathcal{M}$, the KL divergence can be decomposed
% as:

% \begin{align}
% D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1})||p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2}))=\left(D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1})||\mathcal{M})-D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})||\mathcal{M})\right)\nonumber\\
% +D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})||p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1}))
% \end{align}
% where: 
% \begin{itemize}
% \item $D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1})||\mathcal{M})$ is the KL divergence between
% the true distribution $p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1})$ and the best approximation
% within the model class $\mathcal{M}$. 
% \item $D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})||\mathcal{M})$ is the KL divergence between
% the approximating distribution $p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})$ and the best approximation
% within the model class $\mathcal{M}$. 
% \item $D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})||p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1}))$ is the direct KL divergence
% between $p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})$ and $p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1})$. 
% \end{itemize}
% The term $\left(D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1})||\mathcal{M})-D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})||\mathcal{M})\right)$
% captures the discrepancy due to the difference between the true and
% approximating distributions in relation to the model class $\mathcal{M}$.
% This can be seen as the "rest" term or the discrepancy due to model
% misspecification. The last term in the decomposition $D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})||p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1}))$
% captures the "within-model" deviation or the inherent difference
% between the true and approximating distributions without considering
% the model class. This decomposition highlights the two sources of
% error in approximating $p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1})$ with $p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})$:
% the error due to the model misspecification and the inherent error
% between $p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1})$ and $p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})$. If there is no
% model misspecification, then the true data-generating process $p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1})$
% belongs to the model class $\mathcal{M}$. The KL divergence simplifies
% to
% \begin{equation}
% D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1})||p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2}))=D_{KL}(p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{2})||p(\mathbf{y}, \mathbf{x}|(\sigma_s,l)_{1}))
% \end{equation}
% By the classical asymptotic properties of MLE (Maximum Likelihood Estimation) parameters, we know
% that the MLE estimate $\widehat{(\sigma_s,l)}_{i}$ based on sample size $i$ converges (in empirical probability measure $p$ of $i$ samples) to the true parameter $\widehat{(\sigma_s,l)}_{i}\xrightarrow{p}(\sigma_s,l)^{*}$
% with asymptotically normal distribution (converges in distribution $d$) $\sqrt{i}(\widehat{(\sigma_s,l)}_{i}-(\sigma_s,l)^{*})\xrightarrow{d}\mathcal{N}(0,I((\sigma_s,l)^{*})^{-1})$ with the Fisher information matrix $I((\sigma_s,l)^{*})^{-1}$ 
% \cite{schervish2012theory}. 

% When the model is misspecified, there exists a set of parameter
% values, often referred to as \textquotedbl pseudo-true\textquotedbl{}
% parameters, that minimize the KL divergence between the model and
% the true data-generating models. The MLE parameters under misspecification
% will converge to these pseudo-true parameters rather than the true
% parameters (since the true generating model isn't in the considered
% model class) \cite{grunwald2017inconsistency,kleijn2006misspecification}. The MLE parameters can still be asymptotically normal
% (by Bernstein von-Mises Theorem \cite{kleijn2012bernstein,schervish2012theory}), but the limiting distribution is
% centered around the pseudo-true parameters and has a different variance-covariance
% structure than inverse Fisher information matrix $I((\sigma_s,l)^{*})^{-1}$
% in the correctly specified case \cite{schervish2012theory}. Due to misspecification, the
% MLE parameters can exhibit bias even as the sample size grows. This bias is a result of the model's inability to capture certain aspects
% of the true generating model. Our model class $\mathcal{M}$ is the GPR with stationary kernels
% parameterized by kernel parameters $(\sigma_s,l)$ as in \eqref{eq:expK} and \eqref{eq:rbfK}, by looking into the
% the behavior of MLE parameters of stationary kernels we can quantify how
% far it is from the ``stationarity'', which is the rationale of our
% technique. As aforementioned, a stationary kernel will assume that the pairwise covariance does not depend on the location in space, but only on the distance of the input points. This leads us (and others) to deduce that non-stationarity will manifest itself by varying hyperparameters of a stationary kernel --- one isotropic length scale and a constant signal variance  --- when they are trained on localized subsets of the data.



%\review{. We observe empirically that the KL-divergence becomes sensitive to small subsampling when the data-generating mechanism does not belong to the same stationary GP family. This empirical observation motivates our algorithm and works well in practice and the MLE estimate based on subsamples does show non-concentrating distributions for mis-specified models} (See Figure \ref{fig:NS_measure}).  

%\begin{figure}[ht!]
%\centering
%\includegraphics[width=0.3\textwidth]{figures/NS_Gaussian.png}
%\includegraphics[width=0.3\textwidth]{figures/NS_mixGaussian.png}
%\includegraphics[width=0.3\textwidth]{figures/NS_Beta.png}

%\caption{\review{We plot the signal variance-length scale plot for the MLE estimate $(\sigma_s,l)^*$ of GP when the actual data is generated by (left) GP with $(\sigma_{s0},l_0)=(1,1)$ indicated by a red dot (middle) equal mixture of two GP with $(\sigma_{s1},l_1)=(1,1),(\sigma_{s2},l_2)=(5,1)$ (right) Uniform distribution on $[1,10]$ The sample size of the full sample $\mathbf{X},\mathbf{y}$ is 1000, the subsample size $m=100$ and we repeat Algorithm} \ref{alg:NonStationarityCheck} for 100 times. \label{fig:NS_measure}}
%\end{figure}
